Proposal for taking data with the KLOE-2 detector at the DA$\Phi$NE collider upgraded in energy

This document reviews the physics program of the KLOE-2 detector at DA$\Phi$NE upgraded in energy and provides a simple solution to run the collider above the $\phi$-peak (up to 2, possibly 2.5 GeV). It is shown how a precise measurement of the multihadronic cross section in the energy region up to 2 (possibly 2.5) GeV would have a major impact on the tests of the Standard Model through a precise determination of the anomalous magnetic moment of the muon and the effective fine-structure constant at the $M_Z$ scale. With a luminosity of about $10^{32}$cm$^{-2}$s$^{-1}$, DA$\Phi$NE upgraded in energy can perform a scan in the region from 1 to 2.5 GeV in one year by collecting an integrated luminosity of 20 pb$^{-1}$ (corresponding to a few days of data taking) for single point, assuming an energy step of 25 MeV. A few years of data taking in this region would provide important tests of QCD and effective theories by $\gamma\gamma$ physics with open thresholds for pseudo-scalar (like the $\eta'$), scalar ($f_0,f'_0$, etc...) and axial-vector ($a_1$, etc...) mesons; vector-mesons spectroscopy and baryon form factors; tests of CVC and searches for exotics. In the final part of the document a technical solution for the energy upgrade of DA$\Phi$NE is proposed.

==> alpha.tex <==
Precision tests of the Standard Model require an appropriate inclusion
of higher order effects and the knowledge of very precise input parameters.
One of the basic input parameters is the fine-structure constant 
$\alpha$ , determined from the  anomalous 
 magnetic moment of the electron
%\cite{Hanneke:2008tm}
%which depends logarithmically on the energy scale.
 %It has been determined at zero momentum transfer 
 with an impressive accuracy of 0.37 parts per billion 
(ppb)~\cite{Hanneke:2008tm} 
%from the measurement of the anomalous electron
% magnetic moment \cite{Hanneke:2008tm}, 
relying on the validity of 
 perturbative QED~\cite{Gabrielse:2006gg}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%INCLUDE PASSERA
However, physics at nonzero squared momentum transfer $q^2$
is actually described by an effective electromagnetic
coupling $\alpha(q^2)$ rather than by the low-energy
constant $\alpha$ itself. The shift of the fine-structure
constant from the Thomson limit to high energy involves low
energy non-perturbative hadronic effects which spoil this
precision. In particular, the effective fine-structure
constant at the scale $M_{\scriptscriptstyle{Z}}$,
$\alpha(M_{\scriptscriptstyle{Z}}^2) = \alpha/[1-\Delta
\alpha(M_{\scriptscriptstyle{Z}}^2)]$, plays a crucial role
in basic {\small EW} radiative corrections of the {\small
  SM}. An important example is the {\small EW} mixing
parameter $\sin^2 \!\theta$, related to $\alpha$, the Fermi
coupling constant $G_F$ and $M_{\scriptscriptstyle{Z}}$ via
the Sirlin relation~\cite{Sirlin:1980nh,Sirlin:1989uf,Marciano:1980pb}
%
\begin{equation}
  \sin^2 \!\theta_{\scriptscriptstyle{S}} \cos^2 \!\theta_{\scriptscriptstyle{S}} = 
  \frac{\pi \alpha}
{\sqrt 2 G_F M_{\scriptscriptstyle{Z}}^2 (1-\Delta r_{\scriptscriptstyle{S}})},
\label{eq:sirlin}
\end{equation}
%
where the subscript $S$ identifies the renormalisation
scheme. $\Delta r_{\scriptscriptstyle{S}}$ incorporates the
universal correction $\Delta
\alpha(M_{\scriptscriptstyle{Z}}^2)$, large contributions
that depend quadratically on the top quark
mass $m_t$~\cite{Veltman:1977kh} (which led to its indirect determination
before this quark was discovered), plus all remaining
quantum effects.
%
In the {\small SM}, $\Delta r_{\scriptscriptstyle{S}}$
depends on various physical parameters, including
$M_{\scriptscriptstyle{H}}$, the mass of the Higgs boson. As
this is the only relevant unknown parameter in the {\small
  SM}, important indirect bounds on this missing ingredient
can be set by comparing the calculated quantity in
Eq.~(\ref{eq:sirlin}) with the experimental value of $\sin^2
\!\theta_{\scriptscriptstyle{S}}$ (e.g.\ the effective
{\small EW} mixing angle $\sin^2 \!\theta_{\rm eff}^{\rm
  lept}$ measured at LEP and SLC from the
on-resonance asymmetries) once
$\Delta\alpha(M_{\scriptscriptstyle{Z}}^2)$ and other
experimental inputs like $m_t$ are provided. It is important
to note that an error of $\delta
\Delta\alpha(M_{\scriptscriptstyle{Z}}^2) = 35 \times
10^{-5}$~\cite{Burkhardt:2005se} in the effective
electromagnetic coupling constant dominates the uncertainty
of the theoretical prediction of $\sin^2 \!\theta_{\rm
  eff}^{\rm lept}$, inducing an error $\delta(\sin^2
\!\theta_{\rm eff}^{\rm lept}) \sim 12 \times 10^{-5}$
(which is comparable with the experimental value
$\delta(\sin^2 \!\theta_{\rm eff}^{\rm
  lept})^{\scriptscriptstyle \rm EXP} = 16 \times 10^{-5}$
determined by LEP-I and SLD~\cite{leplsd:2005ema,LEPEWWG}) and
affecting the upper bound for $M_H$~\cite{leplsd:2005ema,LEPEWWG,Passera:2008jk}, see Fig.~\ref{fig:blueband}.  Moreover, as
measurements of the effective {\small EW} mixing angle at a
future linear collider may improve its precision by one
order of magnitude, a much smaller value of
$\delta\Delta\alpha(M_{\scriptscriptstyle{Z}}^2)$ will be
required (see below). It is therefore crucial to assess all
viable options to further reduce this uncertainty.
\begin{figure}[ht]
\begin{center}
\includegraphics[width=8cm]{blueband.eps}
\vspace{-1.cm}
\caption{The line is the result of the Electroweak Working Group fit
  using all data~\cite{LEPEWWG}; the band represents an estimate of
  the theoretical error due to missing higher order corrections.  The
  vertical bands show the 95\% CL exclusion limits on
  $M_{\scriptscriptstyle{H}}$ from the direct searches.}
\label{fig:blueband}
\end{center}
\end{figure}
%
The shift $\Delta \alpha(M_{\scriptscriptstyle{Z}}^2)$ can
be split in two parts:
$\Delta\alpha(M_{\scriptscriptstyle{Z}}^2) =
\Delta\alpha_{\rm lep}(M_{\scriptscriptstyle{Z}}^2) + \Delta
\alpha_{\rm had}^{(5)}(M_{\scriptscriptstyle{Z}}^2)$. The
leptonic contribution is calculable in perturbation theory
and known up to three-loop accuracy: $\Delta\alpha_{\rm
  lep}(M_{\scriptscriptstyle{Z}}^2) = 3149.7686\times
10^{-5}$~\cite{Steinhauser:1998rq}. The hadronic contribution $\Delta
\alpha_{\rm had}^{(5)}(M_{\scriptscriptstyle{Z}}^2)$ of the
five light quarks ($u$, $d$, $s$, $c$, and $b$) can be
computed from hadronic $e^+ e^-$ annihilation data via the
dispersion relation~\cite{Cabibbo:1961sz}
%
\begin{equation} 
  \Delta \alpha_{\rm had}^{(5)}(M_{\scriptscriptstyle{Z}}^2) = 
-\left(\frac{\alpha M_{\scriptscriptstyle{Z}}^2}{3\pi}
  \right) \mbox{Re}\int_{m_\pi^2}^{\infty} {\rm d}s 
\frac{R(s)}{s(s- M_{\scriptscriptstyle{Z}}^2
  -i\epsilon)},
\label{eq:delta_alpha_had}
\end{equation}
%
where $R(s) = \sigma^{0}_{\rm had}(s)/(4\pi\alpha^2\!/3s)$ and
$\sigma^{0}_{\rm had}\!(s)$ is the total cross section for $e^+ e^-$
annihilation into any hadronic states, with 
%extraneous {\small QED} and vacuum polarisation 
vacuum polarisation and initial state {\small QED}
corrections subtracted off. The current
accuracy of this dispersion integral is of the order
of 1\%, dominated by the error of the hadronic cross section
measurements in the energy region below a few GeV~\cite{Eidelman:1995ny,Davier:1997kw,Burkhardt:2001xp,Burkhardt:2005se,Jegerlehner:2001wq,Jegerlehner:2003rx,Jegerlehner:2006ju,Jegerlehner:2008rs,Jegerlehner:2003qp,Jegerlehner:2003ip,Hagiwara:2003da,Hagiwara:2006jt}.
%%%END PASSERA%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%
%At the $M_{\scriptscriptstyle{Z}}$ scale the shift of the fine-structure constant 
%involves low energy non-perturbative hadronic effects, which  
%cause a dramatic reduction of accuracy, by several orders of magnitude~\cite{Jegerlehner:2001wq,Jegerlehner:2003rx,Jegerlehner:2006ju,Jegerlehner:2008rs}.
%These low energy strong-interaction effects can be computed from hadronic 
%$e^+e^-$ annihilation data via the dispersion relation~\cite{Cabibbo:1961sz}:
%
%\begin{equation} 
%  \Delta \alpha_{\rm had}^{(5)}(M_{\scriptscriptstyle{Z}}^2) = 
%-\left(\frac{\alpha M_{\scriptscriptstyle{Z}}^2}{3\pi}
%  \right) \mbox{Re}\int_{m_\pi^2}^{\infty} ds 
%\frac{R(s)}{s(s- M_{\scriptscriptstyle{Z}}^2
%  -i\epsilon)},
%\label{eq:delta_alpha_had}
%\end{equation}
%%
%where $R(s) = \sigma^{0}(s)/(4\pi\alpha^2\!/3s)$ and
%$\sigma^{0}\!(s)$ is the total cross section for $e^+ e^-$
%annihilation into hadronic state.

%The current accuracy of this dispersion integral is of the order of 1\%, 
%dominated by the error of the hadronic cross section measurement in the energy region below a few GeV~\cite{Eidelman:1995ny,Davier:1997kw,Burkhardt:2001xp,Burkhardt:2005se,Jegerlehner:2001wq,Jegerlehner:2003rx,Jegerlehner:2006ju,Jegerlehner:2008rs,Jegerlehner:2003qp,Jegerlehner:2003ip,Hagiwara:2003da,Hagiwara:2006jt}.
% This error represents the largest source of the uncertainty of the effective electromagnetic coupling constant,  (recent evaluations give $\Delta\alpha(M^2_Z) = 22\times 10^{-5}$~\cite{Jegerlehner:2008rs,Hagiwara:2006jt}), becoming a limiting factor for the effective electroweak mixing parameter $\sin^2{\theta_f}$, and in turn for the prediction of the Higgs mass~\cite{Collaboration:2008ub}.
Table~\ref{tab:future} (from Ref.~\cite{Jegerlehner:2001wq}) shows that an
uncertainty $\delta \Delta\alpha_{\rm had}^{(5)} \sim 5 \times
10^{-5}$, needed for precision physics at a future linear collider,
requires the measurement of the hadronic cross section with a
precision of $O(1\%)$ from threshold up to the $\Upsilon$ peak.
%
\begin{table}[h]
\begin{center}
 \renewcommand{\arraystretch}{1.4}
 \setlength{\tabcolsep}{1.6mm}
{\footnotesize
\begin{tabular}{|c|c|c|c|}
\hline
$\delta \Delta\alpha_{\rm had}^{(5)} \!\times \! 10^{5} $ 
& $\delta(\sin^2 \!\theta_{\rm eff}^{\rm lept}) \! \times \! 10^{5}$  
& Request on $R$\\
\hline \hline
22   &  7.9 & Present \\
\hline
7   &   2.5 & $\!\delta R/R \sim  1\%$ up to ${J/\psi}$\\
\hline   
5   &   1.8 & $\delta R/R \sim  1\%$ up to $\Upsilon$\\
\hline   
\end{tabular}
}
\caption{\label{tab:future} 
Values of the uncertainties $\delta
\Delta\alpha_{\rm had}^{(5)}$ (first column) and the errors induced by these
uncertainties on the theoretical {\small SM} prediction for $\sin^2
\!\theta_{\rm eff}^{\rm lept}$ (second column). The third column indicates
the corresponding requirements for the $R$ measurement. From Ref.~\cite{Jegerlehner:2001wq}.}
\end{center}
\end{table}

As advocated in~\cite{Jegerlehner:1999hg}, the dispersion integral
(\ref{eq:delta_alpha_had}) can be calculated in a different way: it is
sufficient to calculate $\Delta
\alpha^{(5)}_{\mathrm{had}}(s)$ not directly at $s=M_Z^2$, but at some
much lower scale $s_0=-M_0^2$ in the Euclidean region, which is chosen
such that the difference $\Delta\alpha^{(5)}_{\mathrm{had}}(M_Z^2)-
\Delta \alpha^{(5)}_{\mathrm{had}}(-M_0^2)$ can be reliably calculated
using perturbative QCD (pQCD). In (\ref{eq:delta_alpha_had}) pQCD is
used to compute the high energy tail, including some perturbative
windows at intermediate energies. An extended use of pQCD is
possible by monitoring the validity of pQCD via the Adler function,
essentially the derivative of $\Delta
\alpha^{(5)}_{\mathrm{had}}(s)$ evaluated in the spacelike region:
$\frac{D(Q^2)}{Q^2}=-\frac{3\pi}{\alpha}
\,\frac{d \Delta\alpha_{\mathrm{had}}}{d q^2} |_{q^2=-Q^2}$.
Using a full-fledged state-of-the-art pQCD prediction for the Adler function
one finds that $\Delta\alpha^{(5)}_{\mathrm{had}}(-M_Z^2)-
\Delta \alpha^{(5)}_{\mathrm{had}}(-M_0^2)$ can be neatly calculated from
the predicted Adler function~\cite{Eidelman:1998vc} 
for $M_0 \sim 2.5~\mbox{GeV}$ as a
conservative choice. Also the small missing $\Delta\alpha^{(5)}_{\mathrm{had}}(M_Z^2)-
\Delta \alpha^{(5)}_{\mathrm{had}}(-M_Z^2)$ terms can safely be
calculated in pQCD. The crucial point is that pQCD is used in a fully
controlled manner, away from thresholds and resonances. There are three
points to note: 1) this strategy allows a more precise determination
of $\Delta\alpha^{(5)}_{\mathrm{had}}(M_Z^2)$ than the direct method
based on (\ref{eq:delta_alpha_had}). 2) However, it requires a very
precise QCD calculation and relies on a very precise determination of
the QCD parameters $\alpha_s$, $m_c$ and $m_b$ (for the present status
see \cite{Kuhn:2007vp});
3) Most importantly, the method relies mainly on a precise cross section
measurement in the low energy region, which at the same time is most
important for reducing the uncertainty of the prediction of the muon
$g-2$.  Thus projects like KLOE-2 are absolutely crucial for a better
determination of the effective fine structure constant and the muon
$g-2$ (for details see ~\cite{Jegerlehner:2008rs}).





==> detect.tex <==
Due to the large number of different hadronic channels, a precise
 measurement of the multi-hadronic cross section in the energy below 2 GeV is not a trivial task which demands excellent $\mu/\pi/K$ separation; large acceptance and high multi-track efficiency.

Although a detailed Monte Carlo simulation has not carried out,
the detector hermeticity, the high granularity of the calorimeter, 
the excellent momentum resolution of the drift chamber and the insertion of the inner tracker would characterize KLOE-2 as a proper detector for this kind of
measurement. A clear separation of pions vs charged kaons can be easily 
obtained by the different energy lost in the drift chamber, and by energy-momentum conservation. Precise $\pi/\mu$ separation is more difficult to achieve 
due to the closer mass values, especially at higher energies. 
In this case all the information from the calorimeter 
and drift chamber must be used to kinematically constraint the event. 
Again a detailed Monte Carlo study is here needed to understand if 
KLOE-2 can provide the necessary $\pi/\mu$ separation 
or a dedicated detector upgrade (like the insertion of muon chambers)
is needed.

\noindent
 The beam energy can be determined with an error less than 100 keV
by using  the Compton backscattering (CBS) of laser photons against
 the electron beam. 


==> g-2.tex <==
Like the effective fine-structure constant at the scale
$M_{\scriptscriptstyle{Z}}$, the {\small SM} determination of the
anomalous magnetic moment of the muon $a_\mu$ is presently limited by the
evaluation of the hadronic vacuum polarisation effects, which cannot be 
computed perturbatively at low energies. 
However, using analyticity and unitarity, it was shown
long ago that this term can be computed from hadronic $e^+ e^-$
annihilation data via the dispersion integral~\cite{Gourdin:1969dm}:
%
\begin{eqnarray}
      a_{\mu}^{\mbox{$\scriptscriptstyle{\rm HLO}$}} &=& 
      \frac{1}{4\pi^3}
      \int^{\infty}_{m_{\pi}^2} {\rm d}s \, K(s) \sigma^{0}\!(s) \nonumber \\
                                                                  &=&
      \frac{\alpha^2}{3\pi^2}
      \int^{\infty}_{m_{\pi}^2} {\rm d}s \, K(s) R(s)/s \, .
\label{eq:amu_had}
\end{eqnarray}
%
The kernel function $K(s)$ decreases monotonically with increasing~$s$. This
integral is similar to the one entering the evaluation of the hadronic
contribution $\Delta \alpha_{\rm had}^{(5)}(M_{\scriptscriptstyle{Z}}^2)$ in
Eq.~(\ref{eq:delta_alpha_had}). Here, however, the weight function in the
integrand gives a stronger weight to low-energy data.
A recent compilation of $e^+e^-$ data gives~\cite{Davier:2009zi}:
\begin{equation}
a_\mu^{\scriptscriptstyle{\rm HLO}} = (695.5\pm4.1)\times 10^{-10} \, .
\end{equation}
Similar values are obtained by other
 groups~\cite{Hagiwara:2006jt,Jegerlehner:2008zz,Jegerlehner:2009ry,Eidelman:2009ft}. 


%The fractional accuracy of 0.6\% represents 
%a reduction of more than a factor two of the error respect to 
%8 years ago. 
By adding this contribution to the rest of the
{\small SM} contributions, a recent update of the
 SM prediction of $a_{\mu}$, which uses the hadronic light-by-light
result from~\cite{Prades:2009tw} gives \cite{Davier:2009zi,Prades:2009qp}:
%
\noindent $a_{\mu}^{\mbox{$\scriptscriptstyle{\rm SM}$}}= 116591834 (49)  
\times 10^{-11}$.
%
The difference between the experimental average~\cite{Bennett:2006fi},
$     a_{\mu}^{\mbox{$\scriptscriptstyle{\rm exp}$}}= 11659 2080 (63)  
\times 10^{-11}$
%
and the SM prediction is then
%
$\Delta a_{\mu} = a_{\mu}^{\mbox{$\scriptscriptstyle{\rm exp}$}}-
a_{\mu}^{\mbox{$\scriptscriptstyle{\rm SM}$}} = +246 (80) \times 10^{-11}$,
%
i.e. 3.1 standard deviations (adding all errors in quadrature).
Slightly higher discrepancies are obtained 
%employing the values of the
%leading-order hadronic contribution reported 
in 
Refs.~\cite{Hagiwara:2006jt,Jegerlehner:2009ry,Eidelman:2009ft}.
%
%Recent reviews of the muon $g$$-$$2$ can be found in
%Refs.~\cite{Passera:2004bj, Jegerlehner:2008zz, Jegerlehner:2009ry, Reviews}.
\begin{figure}[ht]
\vspace*{-7mm}
\centering
\includegraphics[height=5cm]{gmdist_c.eps}
\caption{The distribution of contributions (left) and errors (right)
in \% for $a_{\mu}^{\mbox{$\scriptscriptstyle{\rm HLO}$}}$ 
from different energy regions. The error of a
contribution $i$ shown is
$\delta^2_{i\:{\rm tot}}/\sum_i \delta^2_{i\:{\rm tot}}$ in \%. The
total error combines statistical and systematic errors in quadrature. From Ref.~\cite{Jegerlehner:2009ry}}
\label{fig:gmusta}
\end{figure}


As in the case of $\alpha(M^2_Z)$, the uncertainty 
of the theoretical evaluation of
 $a_{\mu}^{\mbox{$\scriptscriptstyle{\rm SM}$}}$
 is still dominated by the  hadronic contribution at low energies,
as shown in Fig.~\ref{fig:gmusta},
 where the region below 2.5 GeV accounts for about 95\% of the squared error to amu, being 55\% the contribution to 
$\delta^2 a^{\rm{HLO}}_{\mu}$ from the region 1 -- 2 GeV.

A reduction of the uncertainty is necessary in order to match 
the increased precision of  the proposed muon g-2 experiments 
at FNAL~\cite{Carey:2009zz} and J-PARC~\cite{Imazato:2004fy}.
 This effort is challenging but possible, and certainly
well motivated by the excellent opportunity the muon $g$$-$$2$ is
providing us to unveil (or constrain) ``new physics'' effects.  Once
again, a long-term program of hadronic cross section measurements at low energies is clearly warranted.


==> g-2_cb.tex <==
Like the effective fine-structure constant at the scale
$M_{\scriptscriptstyle{Z}}$, the {\small SM} determination of the
anomalous magnetic moment of the muon $a_\mu$ is presently limited by the
evaluation of the hadronic vacuum polarisation effects, which cannot be 
computed perturbatively at low energies. 
However, using analyticity and unitarity, it was shown
long ago that the leading order hadronic contribution to $a_{\mu}$,
$a_{\mu}^{\rm HLO}$ can be computed from hadronic $e^+ e^-$
annihilation data via the dispersion integral~\cite{Gourdin:1969dm}:
%
\begin{eqnarray}
      a_{\mu}^{\mbox{$\scriptscriptstyle{\rm HLO}$}} &=& 
      \frac{1}{4\pi^3}
      \int^{\infty}_{m_{\pi}^2} {\rm d}s \, K(s) \sigma^{0}\!(s) \nonumber \\
                                                                  &=&
      \frac{\alpha^2}{3\pi^2}
      \int^{\infty}_{m_{\pi}^2} {\rm d}s \, K(s) R(s)/s \, .
\label{eq:amu_had}
\end{eqnarray}
%
The kernel function $K(s)$ decreases monotonically with increasing~$s$. This
integral is similar to the one entering the evaluation of the hadronic
contribution $\Delta \alpha_{\rm had}^{(5)}(M_{\scriptscriptstyle{Z}}^2)$ in
Eq.~(\ref{eq:delta_alpha_had}). Here, however, the weight function in the
integrand gives a stronger weight to low-energy data.

The contributions to $a_\mu^{\rm HLO}$ and to its uncertainty $\delta
a_\mu^{\rm HLO}$ of the different energy regions
are shown in Fig.~\ref{fig:gmusta}~\cite{Jegerlehner:2009ry}.
The region below 2.5 GeV accounts for about 95\% of the squared uncertainty
$\delta^2 a^{\rm{HLO}}_{\mu}$, 55\% coming 
 from the region 1 -- 2 GeV.
%
\begin{figure}[ht]
\vspace*{-7mm}
\centering
\includegraphics[height=5cm]{gmdist_c.eps}
\caption{The distribution of contributions (left) and errors (right)
in \% for $a_{\mu}^{\mbox{$\scriptscriptstyle{\rm HLO}$}}$ 
from different energy regions. The error of a
contribution $i$ shown is
$\delta^2_{i\:{\rm tot}}/\sum_i \delta^2_{i\:{\rm tot}}$ in \%. The
total error combines statistical and systematic errors in quadrature. From Ref.~\cite{Jegerlehner:2009ry}}
\label{fig:gmusta}
\end{figure}
%

Recently, several papers have been
published~\cite{Hagiwara:2006jt,Davier:2009zi,Jegerlehner:2009ry,Eidelman:2009ft,Prades:2009qp} aiming to extract 
the best overall estimate of the Standard Model (SM) value $a_{\mu}^{\rm
SM}$, including the
evaluation of the $a_\mu^{\rm HLO}$ term based on the 
new measurements of the $e^+e^-$ hadronic cross-sections at low
energy. The resulting estimates are systematically lower than 
the experimental result
$     a_{\mu}^{\mbox{$\scriptscriptstyle{\rm exp}$}}= 11659 2080 (63)  
\times 10^{-11}$ ~\cite{Bennett:2006fi} by an amount between 3 and 3.5
standard deviations. The main contributions to the uncertainty of
$a_{\mu}^{\rm SM}$ are shown in tab.\ref{tab:g-2a} for two estimates~\cite{Davier:2009zi,Jegerlehner:2009ry} based on
different data sets and slightly different theoretical approaches. They are due
to the $a_\mu^{\rm HLO}$ term and to the so called light-by-light
scattering term $a_\mu^{\rm LbL}$~\cite{Prades:2009tw}.
 
In order to clarify the nature of the observed discrepancy between theory
and experiment and eventually
reinforce its statistical significance, 
new direct
measurements of $g-2$ with a factor 4 reduction in uncertainty
have been proposed at Fermilab~\cite{Carey:2009zz} and J-PARC~\cite{Imazato:2004fy}.
With such measurements the uncertainty on the difference $\Delta a_{\mu}$ between the experimental and the
theoretical $a_{\mu}$ will be dominated by the uncertainty on the $e^+e^-$
cross-sections at low energies. The last column of tab.\ref{tab:g-2a} shows
a future scenario based on
realistic improvements in the $e^+e^-$ cross-sections measurements. Such
improvements could be obtained by reducing the uncertainties on the $e^+e^-$
cross-sections from 0.7\% to 0.4\% in the region below 1 GeV and from 6\%
to 2\% in the region between 1 and 2 GeV as shown in tab.\ref{tab:g-2b}.

In this scenario the overall uncertainty on $\Delta a_{\mu}$ could be
reduced by a factor 2. In case the central value remain the same, the
statistical significance will be 6-7 standard deviations.
%
\begin{table}[h]
\begin{center}
 \renewcommand{\arraystretch}{1.4}
 \setlength{\tabcolsep}{1.6mm}
{\footnotesize
\begin{tabular}{|c|c c|c|}
\hline
 & $\delta a_{\mu}$\cite{Jegerlehner:2009ry} & $\delta a_{\mu}$\cite{Davier:2009zi} & $\delta
 a_{\mu}$(prospect) \\
\hline
total & 61 & 49 & 42 \\
\hline
HLO & 53 & 41 & 31 \\
LbL & 39 & 26 & 30 \\
\hline
(exp)-(theo) & 88 & 80 & 45 \\
\hline   
\end{tabular}
}
\caption{\label{tab:g-2a} Estimated uncertainties $\delta a_{\mu}$ in units
$10^{-11}$ according to refs.~\cite{Davier:2009zi,Jegerlehner:2009ry} and
(last column) prospects in case of improved precision in the $e^+e^-$
hadronic cross-section measurement. (Last row) Uncertainty on $\Delta
a_{\mu}$ assuming the present experimental uncertainty of 63 (first two
colums) and an uncertainty of 16 (last column).
}
\end{center}
\end{table}
%
%
\begin{table}[h]
\begin{center}
 \renewcommand{\arraystretch}{1.4}
 \setlength{\tabcolsep}{1.6mm}
{\footnotesize
\begin{tabular}{|c|c|c|c|c|}
\hline
 & $\delta (\sigma)/\sigma$ (\%)present &$\delta a_{\mu}$present
 \cite{Jegerlehner:2009ry} & $\delta (\sigma)/\sigma$ (\%)prospect &$\delta a_{\mu}$prospect  \\
\hline
$\sqrt{s}<1$~GeV & 0.7\% & 33 & 0.4\% & 25 \\
$1<\sqrt{s}<2$~GeV & 6\% & 39 & 2\% & 15 \\
$\sqrt{s}>2$~GeV & & 12 & & 12 \\
\hline
total & & 53 & & 30 \\
\hline
   
\end{tabular}
}
\caption{\label{tab:g-2b} Overall uncertainty on the cross-section
measurement required to get the reduction of uncertainty on $a_{\mu}$ in units
$10^{-11}$ for
three regions of $\sqrt{s}$.
}
\end{center}
\end{table}


 The effort needed to reduce the uncertainties on the $e^+e^-$
cross-sections according to tab.\ref{tab:g-2b} is challenging but possible, and certainly
well motivated by the excellent opportunity the muon $g$$-$$2$ is
providing us to unveil (or constrain) ``new physics'' effects.  Once
again, a long-term program of hadronic cross section measurements at low energies is clearly warranted.


==> gg.tex <==
\begin{figure}[ht]
\centering
\epsfig{file=gg.eps,width=6cm,height=6cm}
\caption{Effective $\gamma\gamma$ luminosity as a function of
 $W_{\gamma\gamma}$ corresponding to an integrated luminosity 
 of  1 fb$^{-1}$ at $\sqrt{s} = m_{\phi}$ (red curve) and at 
$\sqrt{s}$=2.4 GeV (blue curve)}
\label{gg}
\end{figure}

As shown in Fig.~\ref{gg}
The $\gamma\gamma$ physics program at higher energies
 benefit from the larger flux
then at $\phi$ peak with much reduced background. 
In Tab.\ref{ggtab} we report the estimates for the total production rate of 
a pseudoscalar meson (PS) in the process $e^+e^-\rightarrow e^+e^-PS$ 
for three \Dafne\ c.m. energies~\cite{kloe2paper}.

\begin{table}[ht]
\begin{center}
%  \centering
  \caption{\label{ggtab}$e^+e^-\rightarrow e^+e^-PS$ total rate for an integrated
    luminosity of 1 fb$^{-1}$ at three different center of mass energies. No
    tag efficiency is included in the rate calculation.}
%  \protect
%\footnotesize
  \begin{tabular*}{80mm}{c@{\extracolsep{\fill}}cccc}
 %   \toprule
    $\sqrt{s}$ (GeV) & $\pi^0$ & $\eta$ & $\eta'$ \\
    \hline
    1.02 & 4.1$\times 10^5$ & 1.2$\times 10^5$ & 1.9$\times 10^4$ \\
    1.4 & 5.$\times 10^5$ & 2$\times 10^5$ & 1$\times 10^5$ \\
    2.4 & 7.3$\times 10^5$ & 3.7$\times 10^5$ & 3.6$\times 10^5$ \\
    \hline
%\bottomrule
  \end{tabular*}
\end{center}
\end{table}

In addition new higher-mass states become accessible: 
pseudo-scalars 
(like the $\eta'$), scalars ($f_o,f'_o$, etc...) and 
axial-vector ($a_1$, etc...) channels.

%Extending the measurement of $\gamma\gamma \rightarrow \pi\pi$ and 
%$\gamma\gamma \rightarrow \eta\pi$ up to $W_{\gamma\gamma}\,\sim\,1$ GeV, the two-photon width of $f_0(980)$ and $a_0(980)$ can be measured. 
A measurement of the  meson transition form factor for pseudoscalars and axial vector mesons are particularly important 
to get less model-dependent estimations of
the hadronic  light-by-light scattering 
in $(g-2)_{\mu}$~\cite{kloe2paper},
 in a region where few data are available.


==> gg_db.tex <==
The upgrade of the KLOE detector with the installation of four detectors \cite{Babusci:2009sg} 
for electrons and positrons in the final state of the reaction 
\begin{equation}
e^+e^-\to e^+e^-\gamma^*\gamma^*\to e^+e^- X\;,
%\label{eq:gg-stat1}
\end{equation}
gives the opportunity to investigate $\gamma\gamma$ physics at DA$\Phi$NE. This program will 
benefit from the energy upgrade of DA$\Phi$NE not only for the larger $\gamma\gamma$ flux 
(see Fig.~\ref{fig:lumgg}), but also from the opening of channels not avalaible at the $\phi$ peak (like the production of pseudo-scalar
(like the $\eta'$), scalar ($f_0, a_0, f'_0, a'_0$, etc...),
axial-vector ($a_1, f_1, a'_1, f'_1$, etc...), and tensor ($a_2, f_2$, etc...)
 mesons).
\begin{figure}[ht]
\centering
%\epsfig{file=gg.eps,width=6cm,height=6cm}
\includegraphics[height=8cm]{lumgg.eps}
\caption{Effective $\gamma\gamma$ luminosity as a function of
 $W_{\gamma\gamma}$ corresponding to an integrated luminosity 
 of  1 fb$^{-1}$ at $\sqrt{s} = m_{\phi}$ (red curve) and at 
$\sqrt{s}$=2.4 GeV (blue curve)}
\label{fig:lumgg}
\end{figure}

For example, the study of the process in the case in which $X = \pi \pi$ can significantly contributes 
to the solution of the open questions on low--energy hadron physics. This process is a clean probe to 
investigate the nature of the scalar resonance. The nature of the isoscalar scalars seen in $\pi\pi$ 
scattering below 1.6 GeV, namely the $f_0(600)$ or $\sigma$, $f_0(980)$, $f_0(1370)$ and $f_0(1510)$ 
mesons, is still controversial. Various models have been proposed in which some are $\bar{q}q$, some 
$\bar{qq}qq$, sometimes one is a $\bar{K}K$-molecule, and one a glueball \cite{Klempt:2007cp}, but 
definitive statements cannot be drawn. Their two photon couplings will help unraveling the enigma.

The present status of the knowledge about the $\gamma\gamma\to\pi\pi$ is summarized in Fig. \ref{fig:xsects}.
\begin{figure}[htbp]
\begin{center}
\includegraphics[height=7cm]{penn_kloe2.eps}
%\includegraphics[height=5cm]{penn_kloe2.pdf}
\caption{Cross-section results for 
$\,\gamma\gamma\to\pi^+\pi^-\,$ from Mark II \cite{Boyer:1990vu} (below 800
MeV) and Belle \cite{Mori:2006jj} above, integrated over $|\cos \theta^*|\,\le\,0.6$, 
and for $\gamma\gamma\to\pi^0\pi^0$ from Crystal Ball \cite{Marsiske:1990hx} 
below 600 MeV and Belle \cite{Uehara:2008pf} above, integrated over 
$|\cos \theta^*|\,\le\,0.8$. $E$ is the $\gamma\gamma$ c.m. energy. The
curves are from the (as yet) unpublished Amplitude Analysis that includes
the data of Ref. \cite{Uehara:2008pf}.} 
\label{fig:xsects}
\end{center}
\end{figure}
Though the Belle experiment represents an enormous stride in two photon statistics, there is still the possibility 
to make a significant contribution in each of the three energy regions displayed as bands in Fig. \ref{fig:xsects}. Ê
\begin{itemize}
\item[I.] Ê{\bf 850-1100 MeV}: accurate measurement of the $\pi^+\pi^-$ and
$\pi^0\pi^0$ cross-sections (integrated and differential) are crucially
still required, with clean $\mu\mu$ background separation. In addition,
any information just above 1 GeV on $\bar{K}K$ production would
provide an important constraint on the coupled channel Amplitude Analyses
described above. Moreover $\pi^0\eta$ studies will complement the results
from Belle \cite{Uehara:2009cf}. 
\item[II.] {\bf 450-850 MeV}: this is the region where the $\sigma$ pole lies. 
The precision of data in this region is very poor and that allows a range of 
interpretations. Given the importance of the $\sigma$ for our understanding 
of strong coupling QCD and the nature of the vacuum, it is crucial to measure
$\pi\pi$ production in this region in both charge modes.  
\item[III.] {\bf 280-450 MeV}: though this region is essentially controlled by 
the Born contribution it is crucial for the partial wave analyses of the amplitude. 
The Mark II experiment \cite{Boyer:1990vu} is the only one that has made a 
special measurement of the normalised cross-section for the $\pi^+\pi^-$ 
channel near threshold, but the data have very large error-bars. As for the 
neutral channel only the Crystal Ball data \cite{Marsiske:1990hx} are avalaible. 
Also in this case the quality of the data does not  allow any conclusion to be 
drawn about the existence of a resonant-like structure in this region.
\end{itemize}


Single pseudoscalar ($X=\pi^0$, $\eta$ or $\eta^\prime$) production is also accessible and would 
improve the determination of the two--photon decay widths of these mesons, relevant for the measurement 
of the pseudoscalar mixing angle $\varphi_P$, and the measurement of the valence gluon content in the
$\eta^\prime$ wavefunction. Moreover, the study of the same processes gives access to the transition form 
factors $F_{X\gamma^*\gamma^*}(M^2_X,q_1^2,q_2^2)$ at spacelike momentum transfers, that are relevant 
for the hadronic light-by-light scattering contribution to the $g-2$ of the muon \cite{Jegerlehner:2009ry,Prades:2009pn}.


From the experimental point of view, by detecting one electron at large angle with respect to the beams, 
$F_{P\gamma\gamma^*}(M^2_X,Q^2,0)$  with one quasi--real and one virtual spacelike photon ($Q^2=-q^2$) can 
be measured for the on--shell pseudoscalar.  These form factors, as reviewed in Ref. \cite{Dorokhov:2009jd}, have 
been measured by the CELLO \cite{Behrend:1990sr}, CLEO \cite{Gronberg:1997fj} and recently BaBar \cite{Aubert:2009mc} 
collaborations in the range $1<Q^2<40$ GeV$^2$ using single--tagged samples. These data are summarized in 
Fig. \ref{fig:pseudo1}. The region of very low $Q^2$ (less than  0.5 GeV$^2$, the more important for the light-by-light 
scattering contribution, is devoid of experimental data and is the only accessible at DA$\Phi$NE.  By increasing the  
energy of the machine new higher-mass staes will become accessible: pseudoscalars (like the $\eta^\prime$), scalars 
(like the $f_0$) and axial-vector (like $a_1$) mesons. A measurement of all these meson transitions form factors will be of 
fundamental importance to reduce the uncertainties that currently affect the estimates of the hadronic LbL scattering. 
\begin{figure}[htb]
\begin{tabular}{ccc}
\resizebox{.3\textwidth}{!}{\includegraphics{fpi.eps}} & 
\resizebox{.3\textwidth}{!}{\includegraphics{feta.eps}} & 
\resizebox{.3\textwidth}{!}{\includegraphics{fetapr.eps}} \\
%\resizebox{.3\textwidth}{!}{\includegraphics{fpi.pdf}} & 
%\resizebox{.3\textwidth}{!}{\includegraphics{feta.pdf}} & 
%\resizebox{.3\textwidth}{!}{\includegraphics{fetapr.pdf}} \\
\end{tabular}
\caption{Left: the $\pi^0$ transition form factor as measured
by the CELLO, CLEO and BaBar experiments. The curve showing an asymptotic 
limit at 160 MeV is from CLEO parametrization \cite{Gronberg:1997fj} 
while the other is from the $\mathcal{F}_{\pi\gamma\gamma^*}(m^2_P,Q^2,0)$ 
expression given in Ref. \cite{Dorokhov:2009jd}. Center: the $\eta$ transition 
form factor as measured by CELLO and by CLEO in the specified 
$\eta$ decay channels.
Right: the $\eta^\prime$ form factor as measured by CELLO and by CLEO in the 
specified $\eta^\prime$ decay channels. The curves in the central and 
left panel  
represent the CLEO parametrization 
for the form factors \cite{Gronberg:1997fj}.}
\label{fig:pseudo1}
\end{figure}



==> intro.tex <==
In this section we discuss the physics program that can be achieved 
by running DA$\mathrm{\Phi}$NE outside the $\phi$ meson peak (so called DA$\mathrm{\Phi}$NE-2 program in the following).
We consider a maximum energy of $\sqrt{s}=2.5$ GeV, with a luminosity of $\sim$10$^{32}$cm$^{-2}$s$^{-1}$, already exceeded by far by DA$\mathrm{\Phi}$NE at the $\phi$ peak.
With such a machine one can easily collect an integrated luminosity of 
 about 5 fb$^{-1}$ between 1 and 2.5 GeV in a few years of data taking.
This high statistics,  much larger than that collected at
 any previous machine in this energy range, 
will represent a major improvement in physics at these energies, with 
relevant implications for the precision tests of the Standard Model, like the  
$g-2$ of the muon and the effective fine-structure constant at the $M_Z$ scale 
 $\alpha_{em}(M^2_Z)$. The only direct competitor project is VEPP-2000 at Novosibirsk, %\cite{VEPPtot} 
which will cover
the center-of-mass energy range between 1 and 2 GeV with two experiments. This
project is expected to start by year 2010 with a luminosity ranging between 
$10^{31}$cm$^{-2}$s$^{-1}$ at 1 GeV and 
$10^{32}$cm$^{-2}$s$^{-1}$ at 2 GeV.
Other ``indirect'' competitors are the higher
energy $e^+e^-$ colliders ($\tau$-charm and B-factories) that in principle
cover the DA$\mathrm{\Phi}$NE-2 energy range by means of radiative return.
However, due to the photon emission, as we will show later, 
the ``equivalent'' luminosity produced by these machines
 in the region between 1 and 2.5 GeV is
much less than the one expected by DA$\mathrm{\Phi}$NE-2 
%(20 pb$^{-1}$ per point).

In the following subsections we present the main physics motivations for this
 off-peak program.
 We start with the implication for precision tests of the Standard Model
from a precise measurement 
 of the multi-hadronic cross sections in the energy region below 2.5 GeV.
%, and its
%implication for precision tests of the Standard Model
 %for $e^+e^-$ $\to$ {\it hadrons} in a very wide center-of-mass 
%energy range, from the
%$\pi\pi$ threshold up to 2.5 GeV, and its implications for precision
%tests of the Standard Model.
% ~(\ref{subsubsec:SMTESTS}), and vector meson
%spectroscopy ~(\ref{Vecto}).
%We finally describe the physics potential of 
%$\gamma\gamma$ collision studies.
%~(\ref{Gamma}). 
%Finally we discuss also the subjects
%of the hadron form factors ~(\ref{Bario}) and of the kaon-nucleus interactions
%~(\ref{Kaons}).   
%\subsection{The Hadronic Contribution to (g-2)$_\mu$ and $\alpha_{em}$}
%\label{sec:g-2had}
%


==> search.tex <==
In the last years 
recent astrophysical puzzles [Pamela, Actic, Fermi, etc...] and the
long-standing Dark Matter problem, have motivated the
construction of various exotic extensions of the SM model
characterized by:
\begin{itemize}
\item[-] new light states [vectors and scalars with masses in the 0.1 - 1
GeV range];
\item[-] weakly coupled to photons, or directly coupled to muons and/or
electrons.\\
\end{itemize}
Precision differential measurements of $e^+e^-\to e^+e^-+\gamma$ 
and/or  $e^+e^-\to \mu^+\mu^-+\gamma$  
and/or $e^+e^-\to E_{missing}+\gamma$ at low energies are the best way to
constrain (or find evidences...) of such models (large parameter
space is still unexplored)~\cite{kloe2paper}. 
A dedicated study has already started at KLOE.


==> spec.tex <==
Cross sections of exclusive final states are also
important for spectroscopy of vector mesons, whose properties provide
fundamental information on interactions of light quarks. 
PDG lists the following vectors between 1 and 2~GeV~\cite{Yao:2006px}: 
$\omega(1420)$, $\rho(1450)$, $\omega(1650)$, $\phi(1680)$, and
$\rho(1700)$.
However, even their basic parameters ($M,~\Gamma,~\Gamma_{ee}$)
are  badly known. In addition many states still needed a confirmed
 identification.
As discussed in~\cite{kloe2paper}
 there are still many puzzles and unknown things;
 some progress  can be achieved in ISR studies at BaBar and Belle, but 
such analyses are statistically limited, and  a real
breakthrough can happen at the dedicated colliders like
DA$\mathrm{\Phi}$NE-2.
{\bf something on BFF}

